SynBench: Task-Agnostic Benchmarking of Pretrained Representations using Synthetic Data

Recent success in fine-tuning large models, that are pretrained on broad data at scale, on downstream tasks has led to a significant paradigm shift in deep learning, from task-centric model design to task-agnostic representation learning and task-specific fine-tuning. As the representations of pretrained models are used as a foundation for different downstream tasks, this paper proposes a new task-agnostic framework, \textit{SynBench}, to measure the quality of pretrained representations using synthetic data. We set up a reference by a theoretically-derived robustness-accuracy tradeoff of the class conditional Gaussian mixture. Given a pretrained model, the representations of data synthesized from the Gaussian mixture are used to compare with our reference to infer the quality. By comparing the ratio of area-under-curve between the raw data and their representations, SynBench offers a quantifiable score for robustness-accuracy performance benchmarking. Our framework applies to a wide range of pretrained models taking continuous data inputs and is independent of the downstream tasks and datasets. Evaluated with several pretrained vision transformer models, the experimental results show that our SynBench score well matches the actual linear probing performance of the pre-trained model when fine-tuned on downstream tasks. Moreover, our framework can be used to inform the design of robust linear probing on pretrained representations to mitigate the robustness-accuracy tradeoff in downstream tasks.

==> SynBench arxiv/CP_Conclusion.tex <==
\section{Discussion and Conclusion}

In this paper, we propose a new \textbf{task-agnostic} framework \textit{SynBench} for benchmarking the robustness-accuracy performance of pretrained representations.
SynBench is fundamentally task-independent and provides a quantifiable score that does not reply on any real-life data.
SynBench exploits an idealized data distribution, class conditional Gaussian mixture, to establish a theoretically-derived robustness-accuracy tradeoff, which serves as the reference for pretrained representations. 
Finally, a quantifiable score \textit{SynBench-Score} is provided that compares the ratio of area-under-curve between the reference and the pretrained representations. 
We validate the usefulness of SynBench on several pretrained vision transformers in giving insightful comparisons on different model attributes (e.g. model size, fine-tuned pretraining representations, ViT patch size, linear probing).

While we delved into the robustness-accuracy performance of pretrained representations of vision transformers, we envision the SynBench framework to be further extended to other trustworthiness dimensions such as privacy, fairness, etc. Moreover, as the popularization of pretrained representations in various domains (e.g. vision, language, speech),  we foresee SynBench to be generalized to more domains, and shed light on task-agnostic benchmarking designs.

==> SynBench arxiv/CP_Experiment.tex <==
\section{Experimental Results}
\begin{table}[t]
    \centering
    \begin{tabular}{c|ccccccc}
    Model & Arch. & pretraining  & fine-tuning  & patch & \# parameters (M)\\\hline
    % SimCLR-ResNet18 & ResNet18 & Imgn1k & No-SimCLR & No & Adam\footnote{We don't distinguish the variants of Adam.} & NA\\
    % SimCLR-ResNet50 & ResNet50 & Imgn1k & No-SimCLR & No & Adam & NA\\
    % DINO-ResNet50 & ResNet50 & Imgn1k & No-DINO & No & NA\\
    % DINO-ViT-B & ViT-Base & Imgn1k & No-DINO & No & 16 \\
    ViT-Ti/16 & ViT-Tiny & Imgn21k & Imgn1k & 16 & 5.7\\
    ViT-B/16 & ViT-Base & Imgn21k & Imgn1k & 16 & 86.6\\
    ViT-B/16-in21k & ViT-Base & Imgn21k & No & 16 & 86.6\\
    % ViT-B/8 & ViT-Base & Imgn21k & Imgn1k & 8 & 86.6\\
    ViT-B/32 & ViT-Base & Imgn21k & Imgn1k & 32 & 88.2\\
    ViT-L/16 & ViT-Large & Imgn21k & Imgn1k & 16 & 304.3\\\hline
   Variation:&\\
    Model size& \multicolumn{4}{l}{(ViT-Ti/16, ViT-Base/16, ViT-Large/16)}\\
    % ResNet vs ViT& \multicolumn{5}{l}{(DINO-ResNet50, DINO-ViT-B)}\\
    Finetuning& \multicolumn{4}{l}{ (ViT-B/16, ViT-B/16-in21k)}\\
    ViT patch size& \multicolumn{4}{l}{(ViT-B/16, ViT-B/32)}\\
    \end{tabular}
    \caption{Model descriptions.}
    \label{tab:models_comparison}
\end{table}
\begin{table}[t]
    \centering
    \scalebox{0.9}{
    \begin{tabular}{c|ccccc|ccc}
    $a_t=0.7$ & $\epsilon=0$ & $\epsilon=0.2$ & $\epsilon=0.4$ & $\epsilon=0.6$ & $\epsilon=0.8$ & CIFAR10 & CIFAR10-c %& Food
    \\\hline
    ViT-B/16 & 0.33 & 0.37 & 0.32 & 0.20 & 0.06 & 95.0 & 81.2 %& 80.1
    \\
    ViT-B/16-in21k & 0.20 & 0.23 & 0.18 & 0.07 & 0.01 & 89.6 & 71.4 %& 76.3
    \end{tabular}}
    \caption{Comparisons on the finetuning procedure in pretraining. We report the SynBench-Score of ViTs with or without finetuning pretrained representations, and the standard linear probing accuracy on CIFAR10 and transfer accuracy on CIFAR10-c.}
    \label{tab:finetune}
\end{table}
\begin{table}[h!]
    \centering
    \scalebox{0.9}{
    \begin{tabular}{c|c|ccccc|ccc}
    % ta$=0.6$ & $\epsilon=0$ & $\epsilon=0.2$ & $\epsilon=0.4$ & $\epsilon=0.6$ & $\epsilon=0.8$ & Max & CIFAR10 & CIFAR10-c & Food\\
    % ViT-Ti/16 & 0.14 & 0.13 & 0.11 & 0.09 & 0.07 & 0.14 & 81.9 & 60.3 & 53.2\\
    % ViT-B/16 & 0.45 & 0.47 & 0.44 & 0.36 & 0.25 & 0.47 & 95.0 & 81.9 & 80.1\\
    % ViT-L/16 & 0.38 & 0.43 & 0.41 & 0.35 & 0.25 & 0.43 & 98.0 & 90.7 & 87.0\\
    % ta$=0.65$ & $\epsilon=0$ & $\epsilon=0.2$ & $\epsilon=0.4$ & $\epsilon=0.6$ & $\epsilon=0.8$ & Max & CIFAR10 & CIFAR10-c & Food\\
    % ViT-Ti/16 & 0.05 & 0.04 & 0.02 & 0.01 & 0 & 0.05 & 81.9 & 60.3 & 53.2\\
    % ViT-B/16 & 0.39 & 0.42 & 0.38 & 0.28 & 0.15 & 0.42 & 95.0 & 81.9 & 80.1\\
    % ViT-L/16 & 0.32 & 0.38 & 0.36 & 0.29 & 0.17 & 0.38 & 98.0 & 90.7 & 87.0\\
    $a_t$ & Model & $\epsilon=0$ & $\epsilon=0.2$ & $\epsilon=0.4$ & $\epsilon=0.6$ & $\epsilon=0.8$ & CIFAR10 & CIFAR10-c %& Food
    \\\hline
    \multirow{3}{*}{$0.7$} & ViT-Ti/16 & 0.01 & 0 & 0 & 0 & 0 & 81.9 & 59.1 %& 53.2
    \\
    & ViT-B/16 & 0.33 & 0.37 & 0.32 & 0.20 & 0.06 & 95.0 & 81.2 %& 80.1
    \\
    & ViT-L/16 & 0.26 & 0.33 & 0.30 & 0.22 & 0.11 & 98.0 & 90.3 %& 87.0
    \\\hline
    \multirow{3}{*}{$0.75$} & ViT-Ti/16 & 0 & 0 & 0 & 0 & 0 & 81.9 & 59.1 %& 53.2
    \\
    & ViT-B/16 & 0.26 & 0.30 & 0.25 & 0.11 & 0.01 & 95.0 & 81.2 %& 80.1
    \\
    & ViT-L/16 & 0.19 & 0.27 & 0.24 & 0.16 & 0.04 & 98.0 & 90.3 %& 87.0
    \\\hline
    \multirow{3}{*}{$0.8$} & ViT-Ti/16 & 0 & 0 & 0 & 0 & 0 & 81.9 & 59.1 %& 53.2
    \\
    & ViT-B/16 & 0.19 & 0.23 & 0.17 & 0.04 & 0 & 95.0 & 81.2 %& 80.1
    \\
    & ViT-L/16 & 0.12 & 0.21 & 0.18 & 0.09 & 0 & 98.0 & 90.3 %& 87.0
    \\\hline
    \multirow{3}{*}{$0.85$} & ViT-Ti/16 & 0 & 0 & 0 & 0 & 0 & 81.9 & 59.1 %& 53.2
    \\
    & ViT-B/16 & 0.10 & 0.15 & 0.09 & 0 & 0 & 95.0 & 81.2 %& 80.1
    \\
    & ViT-L/16 & 0.05 & 0.13 & 0.10 & 0.03 & 0 & 98.0 & 90.3 %& 87.0
    \\\hline
    \multirow{3}{*}{$0.9$} & ViT-Ti/16 & 0 & 0 & 0 & 0 & 0 & 81.9 & 59.1 %& 53.2
    \\
    & ViT-B/16 & 0.02 & 0.04 & 0.01 & 0 & 0 & 95.0 & 81.2 %& 80.1
    \\
    & ViT-L/16 & 0 & 0.04 & 0.03 & 0 & 0 & 98.0 & 90.3 %& 87.0
    \end{tabular}}
    \caption{Comparisons on the model sizes. The SynBench-Score of ViTs of different sizes, and the standard linear probing accuracy on CIFAR10 and transfer accuracy on CIFAR10-c.}
    \label{tab:model_size}
\end{table}

% We start our discussion in the following few aspects. In Section~\ref{subsec:verify_attack}, we demonstrate the correlation of our SynBench bounds with widely-adopted adversarial attack upper bounds. In Section~\ref{subsec:model_zoo}, we apply SynBench on various pretrained representation networks to gauge how pretrining attributes might affect the performance. 

% \subsection{SynBench vs. autoattack bound on real data}
% \label{subsec:verify_attack}
% In this experiment, we use CIFAR10~\citep{krizhevsky2009learning} to generate 45 binary downstream classification tasks (10 classes, 10 choose 2). Furthermore, to validate SynBench's behavior under more diverse data manifold, we also use the first ten classes of Food-101~\citep{bossard14} to generate another 45 binary downstream classification tasks. 

% We propagate the real-life data through a ResNet18 trained by SimCLR~\citep{chen2020simple} and obtain the SynBench scaled bound in representation space with the help of Result~\ref{thm:rep_bound}. To confirm the validity of the robustness-accuracy tradeoff implied by SynBench, we further perform AutoAttack~\citep{croce2020reliable} in the raw data space and scale the average attack bounds by the attack bound of the mediod point. Specifically, the mediod point of a class is the class sample that has a representation that is closest to the mean of all class representations, i.e. $x = \argmin_{x\in\{x_i, y_i\}} f_\theta(x)$

% \textcolor{red}{show the autoattack results, now running food attacks again due the inconcsistency of the train/test transformation -> remove it for workshop submission}

% \subsection{Probing the model zoo}
% \label{subsec:model_zoo}
In this experiment, we exemplify the use of SynBench given a pretrained representation network. In order to compare among network attributes, it is desirable to control the variates. In Table~\ref{tab:models_comparison}, we list severeal pretrained vision transformers (ViTs)\footnote{https://github.com/rwightman/pytorch-image-models}\citep{dosovitskiy2020image,chen2021vision} and make comparisons to our best knowledge. We note that the performance of these models might be nuanced by scheduler, curriculum, and training episodes, which are not captured in the above table. To provide a comprehensive evaluation, we give SynBench-Score$(\theta,\epsilon,a_{t})$ with $a_t$ ranging from 0.7 to 0.9, and $\epsilon$ from 0 to 0.8. Due to space limit, some $a_t$ results are deferred to the appendix.

% With different prefix in Table~\ref{tab:models_comparison} model names, they correspond to different model sources: DINO-\footnote{https://github.com/facebookresearch/dino}\citep{caron2021emerging}, 
% DeiT-\footnote{https://github.com/facebookresearch/deit}\citep{touvron2021training}, 
% ViT-\footnote{https://github.com/rwightman/pytorch-image-models}\citep{dosovitskiy2020image,chen2021vision}.

Apart from the task-agnostic metrics SynBench-Score developed in this paper, we also report linear probing accuracy on CIFAR10 and CIFAR10-c~\citep{hendrycks2019robustness} to validate the standard and transfer accuracy (use the probing layer trained on CIFAR10 to probe CIFAR10-c). We emphasize that SynBench-Score offers a quantifiable score for robustness-accuracy performance benchmarking and is intrinsically a task-agnostic evaluation of the pretrained model. Therefore, although SynBench-Score may share trends with empirical real-life tasks (e.g. CIFAR10), it is meant to characterize a general behavior of the pretrained representations.

% \begin{table}[t]
%     \centering
%     \begin{tabular}{c|cccccc}
%     Model & Arch. & pretraining & Supervised & fine-tuning & optimizer & patch\\\hline
%     % SimCLR-ResNet18 & ResNet18 & Imgn1k & No-SimCLR & No & Adam\footnote{We don't distinguish the variants of Adam.} & NA\\
%     % SimCLR-ResNet50 & ResNet50 & Imgn1k & No-SimCLR & No & Adam & NA\\
%     DINO-ResNet50 & ResNet50 & Imgn1k & No-DINO & No & Adam & NA\\
%     DINO-ViT-B & ViT-Base & Imgn1k & No-DINO & No & Adam & 16 \\
%     DeiT-B & DeiT-Base & Imgn1k & Yes & No & Adam & 16\\
%     ViT-B/16 & ViT-Base & Imgn21k & Yes & Imgn1k & Adam & 16\\
%     ViT-B/16-in21k & ViT-Base & Imgn21k & Yes & No & Adam & 16\\
%     ViT-B/16-sam & ViT-Base & Imgn1k & Yes & No & Sam & 16\\
%     % ViT-B/16-gsam & ViT-Base & Imgn1k & Yes & No & gsam & 16\\
%     % ViT-B/8 & ViT-Base & Imgn21k & Yes & Imgn1k & Adam & 8\\
%     ViT-B/32 & ViT-Base & Imgn21k & Yes & Imgn1k & Adam & 32\\
%     ViT-L/16 & ViT-Large & Imgn21k & Yes & Imgn1k & Adam & 16\\
%     ViT-Ti/16 & ViT-Tiny & Imgn21k & Yes & Imgn1k & Adam & 16\\\hline
%     Compare:&\\
%     Model size& \multicolumn{6}{l}{(ViT-Ti/16, ViT-Base/16, ViT-Large/16)}\\
%     % DINO vs SimCLR& \multicolumn{6}{l}{(SimCLR-ResNet50, DINO-ResNet50)}\\
%     ResNet vs ViT& \multicolumn{6}{l}{(DINO-ResNet50, DINO-ViT-B)}\\
%     % Self-vs supervised& \multicolumn{6}{l}{(DINO-ViT-B, \textcolor{red}{DeiT-B})}\\
%     Finetuning& \multicolumn{6}{l}{ (ViT-B/16, ViT-B/16-in21k)}\\
%     ViT patch size& \multicolumn{6}{l}{(ViT-B/16, ViT-B/32)}\\
%     Optimizer& \multicolumn{6}{l}{(DeiT-B, ViT-B/16-sam)}
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:models_comparison}
% \end{table}
\textbf{Fine-tuned pretraining representation.}
When applying a pretrained representation network to the desired task, one can either only train a linear head on top of a fixed pretrained model, or perform fine-tuning of both the representation network and the linear head.
Thus, in Table~\ref{tab:finetune}, we investigate how the fine-tuning process is affecting the representation networks. Specifically, both networks in Table~\ref{tab:finetune} is pretrained on Imagenet 21k with supervision. After the pretraining, ViT-B/16 is further finetuned on Imagenet 1k. Interestingly, SynBench-Score shows that this finetuning is beneficial as improvements are witnessed across all $\epsilon$ with SynBench-Score, which well match the empirical observation give by CIFAR10 and CIFAR10-c and prior results~\citep{kumar2021fine}.

\textbf{Model size.}
\begin{table}[t]
    \centering
    \scalebox{0.9}{
    \begin{tabular}{c|ccccc|ccc}
    $a_t=0.6$ & $\epsilon=0$ & $\epsilon=0.2$ & $\epsilon=0.4$ & $\epsilon=0.6$ & $\epsilon=0.8$ & CIFAR10 & CIFAR10-c 
    \\\hline
    % ViT-B/8 & 0.54 & 0.56 & 0.54 & 0.50 & 0.43 & 93.7 & 79.5 & 81.8\\
    ViT-B/16 & 0.45 & 0.47 & 0.44 & 0.36 & 0.25 & 95.0 & 81.2
    \\
    ViT-B/32 & 0.02 & 0.03 & 0.03 & 0.01 & 0 & 92.2 & 76.6 
    \end{tabular}}
    \caption{Comparisons on the ViT patch size. The SynBench-Score of ViTs of different patch sizes, and the standard linear probing accuracy on CIFAR10 and transfer accuracy on CIFAR10-c. The Imagenet result shows an average accuracy over 6 Imagenet variants.}
    \label{tab:patchsize}
\end{table}
\begin{table}[t]
    \centering
    \scalebox{0.9}{
    \begin{tabular}{c|ccccc}
       & $\argmax_\epsilon$ & \multicolumn{1}{c}{$\Delta$ robust linear probing} & \\\cline{3-4}
       & SynBench-Score & mean (CIFAR10,CIFAR10-c) &\\\hline
       ViT-Ti/16 & 0 & 70.5\textcolor{blue}{\textbf{+0}} &\\
       ViT-B/16 & 0.2 & 88.1\textcolor{blue}{\textbf{+0.5}}  \\
       ViT-L/16 & 0.2 & 94.2\textcolor{blue}{\textbf{+0.6}} \\
       ViT-B/16-in21k & 0.2 & 80.5\textcolor{blue}{\textbf{+0.5}} \\
       % ViT-B/8 & 0.2 & 86.6\textcolor{blue}{\textbf{-0.9}}\\
       ViT-B/32 & 0.2 & 84.4\textcolor{blue}{\textbf{-0.1}} 
    \end{tabular}}
    \caption{CIFAR10 and CIFAR10-c accuracy \textcolor{blue}{changes} using $\epsilon$-robust linear probing with $\epsilon=\argmax_\epsilon$SynBench-Score.}
    \label{tab:advtrain}
\end{table}
In Table~\ref{tab:model_size}, we compare ViTs of different sizes. Specifically, we perform SynBench on ViT-Tiny, ViT-Base, and ViT-Large with patch size being 16. 
% Besides SynBench, we also report Avg. Max $a$ as introduced in Section\ref{subsec:metrics}. 
% We give SynBench-Score$(\theta,\epsilon,a_{t})$ with $a_t$ ranging from 0.7 to 0.9. 
The model parameter $\theta$ is provided by the pretrained model. It is noticeable that ViT-B/16 is generally on par with ViT-L/16. When we set the threshold accuracy to be higher values, ViT-L/16 starts to give slightly better evaluations especially with larger $\epsilon$. One interesting observation is that for each model, SynBench score is not necessarily monotonic in $\epsilon$, which indicates standard linear probing (i.e., $ \epsilon=0$) may not be the most effective way to probing pretrained representations in terms of robustness-accuracy performance, which is consistent with recent findings \citep{fan2021does}. See the ``Robust linear probing'' paragraph below for detailed analysis.
We also observe that larger models exhibit better resilience (slower reduction in SynBench score) as $\epsilon$ increases.
% The Avg. Max $a$ in this experiment is monotonically increasing with the model size, suggesting larger models has more potential to yield higher standard accuracy.


\textbf{ViT patch size.}
We also compare vision transformer patch sizes in Table~\ref{tab:patchsize}. Specifically, we give ViT-Base with patch size being 16 and 32, individually. 
SynBench-Scores show an consistent trend as the model performance on CIFAR10 and CIFAR10-c.
% Besides CIFAR10 and CIFAR10-c accuracy, we also list an average Imagenet results that are available online\footnote{https://github.com/rwightman/pytorch-image-models/tree/master/results}. Specially, 6 Imagenet variants are considered including ImageNet Validation~\citep{russakovsky2015imagenet}, Real Labels~\citep{beyer2020we}, (clean) Adversarial~\citep{hendrycks2021natural}, and (clean) Rendition~\citep{hendrycks2021many}. We defer the full table of their results to the appendix. 

% \subsubsection{Optimizer}
% \begin{table}[h!]
%     \centering
%     \scalebox{0.8}{
%     \begin{tabular}{c|ccccccccc}
%     ta$=0.7$ & $\epsilon=0$ & $\epsilon=0.2$ & $\epsilon=0.4$ & $\epsilon=0.6$ & $\epsilon=0.8$ & Avg. Max $a$ & CIFAR10 & CIFAR10-c & Food\\
%     DeiT-B & 0 & 0 & 0 & 0 & 0 & 0 & 95.7 & 85.3 & 78.0\\
%     ViT-B/16-sam & 0.79 & 0.87 & 0.84 & 0.78 & 0.67 & 0.87 & 94.9 & 81.5 & 75.7
%     \end{tabular}}
%     \caption{Optimizer}
%     \label{tab:ta0.7}
% \end{table}

% Question: we can't tell from this table that Sam optimizer is better, suspect it is because of the Deit implementation. Shall we remove this for workshop submission and look for ViT imgnt1k for iclr?

\textbf{Robust linear probing.}
According to Table~\ref{tab:model_size}, $0.2$-robust Bayes classifiers consistently give better scores compared to $0$-robust (standard) Bayes classifiers with ViT-B/16 and ViT-L/16. 
This offers us a quick way of gauging the suitable downstream robust probing parameter for the given pretrained model.
We stipulate that observing a $0.2$-robust Bayes classifier to yield better SynBench-Score than a $0$-robust Bayes classifier may suggest the pretrained network to produce representations that have better overall performance with linear classifiers trained by $0.2$-robust linear probing. We validate this by performing robust linear probing on representations rendered by ViTs for CIFAR10 classifications. Results are shown in Table~\ref{tab:advtrain}. For a given pretrained model, let $f$ and $g$ be the pretrained network and linear probing layer, we solve the optimization problem $\min_{g}\max_{\|\delta\|\leq \epsilon} L(g(f(x+\delta)),y)$ using the PyTorch library Torchattacks\footnote{https://github.com/Harry24k/adversarial-attacks-pytorch} and 10-step PGDL2 attacks~\citep{madry2018towards} for adversarial training.
From Table~\ref{tab:advtrain}, we see that robust linear probing with $\epsilon=\argmax_\epsilon$SynBench-Score generally gives a decent robustness-accuracy tradeoff.
For example, with robust linear probing, we obtain a $1.3\%$ increase in CIFAR10-c transfer accuracy at the cost of $0.4\%$ drop in CIFAR10 accuracy with ViT-B/16 (as in Table~\ref{tab:full_advtrain}). A more complete table on $\epsilon$-robust linear probing results with different $\epsilon$ is given in the appendix.

% \jeet{Write the final experimental results out more clearly. Need to highlight the performance difference between $0$-robust classifier and the $0.2$-robust classifier trained on CIFAR10 and CIFAR10-c.}


% \paragraph{ResNet vs ViT.}
% \begin{table}[h!]
%     \centering
%     \scalebox{0.8}{
%     \begin{tabular}{c|cccccc|ccc}
%     $a_t=0.7$ & $\epsilon=0$ & $\epsilon=0.2$ & $\epsilon=0.4$ & $\epsilon=0.6$ & $\epsilon=0.8$ & Avg. Max $a$ & CIFAR10 & CIFAR10-c & Food\\\hline
%     DINO-ResNet50 & 0.39 & 0.66 & 0.61 & 0.57 & 0.52 & 97.1 & 92.8 & 73.0 & 78.8\\
%     DINO-ViT-B & 0.55 & 0.59 & 0.55 & 0.48 & 0.36 & 95.9 & 96.3 & 79.9 & 79.4
%     \end{tabular}}
%     \caption{Comparisons on model types - ResNet vs. ViT.}
%     \label{tab:networtype}
% \end{table}

% In Table~\ref{tab:networtype}, we compare pretrained models based on the residual network~\citep{he2016deep} and vision transformer~\cite{dosovitskiy2020image}. Both representation networks are obtained from the same source and trained by DINO~\citep{caron2021emerging} in a self-supervised learning fashion. When $\epsilon=0$ (i.e. a standard Bayes classifier), DINO trained vision transformer gives a score of 0.55, surpassing DINO trained ResNet50's 0.39. For $\epsilon=0.2$-$0.8$, DINO-ResNet50 scores higher than DINO-ViT in our robustness-accuracy performance benchmarking. 



==> SynBench arxiv/CP_Introduction.tex <==
\section{Introduction}
%With the advancement of machine learning research, bigger and larger models were trained and deployed for numerous real-world applications. Despite being powerful, many models were empowered by considerable amount of data, and training such models were both power-intensive and time-consuming.
%To reduce the burden, more efforts have been put in recent years to study models that can be reused with minimal fine-tuning. Specifically, instead of learning task and data specific networks, representation networks are trained to be used for different tasks and data.

In recent years, the use of large pretrained neural networks for efficient fine-tuning on downstream tasks has prevailed in many application domains such as vision, language, and speech. Instead of designing task-dependent neural network architectures for different downstream tasks, the current methodology focuses on the principle of task-agnostic pretraining  and task-specific finetuning, which uses a neural network pretrained on a large-scale dataset (often in a self-supervised or unsupervised manner) to extract generic representations of the input data, which we call \textit{pretrained representations} for simplicity. The pretrained representations are then used as a foundation \citep{bommasani2021opportunities} to solve downstream tasks by training a linear head (i.e., linear probing) on the data representations with the labels provided by a downstream dataset, or by simply employing zero-shot inference. Moreover, to handle multi-modal data, one can use a similar neural network architecture (e.g., transformer) for multi-modal data representation learning and alignment.
Successful examples following this new machine learning paradigm include the GPT-3 language model \citep{brown2020language}, the vision transformer \citep{arnab2021vivit}, and the CLIP image-text model \citep{radford2021learning},  to name a few.     


As large pretrained models are shown to achieve state-of-the-art performance on a variety of downstream tasks with minimal fine-tuning, 
%while their development and training costs bring about immense expense in computation resources, 
there is an intensified demand for using pretrained representations from a large model for efficient finetuning. However, if the underlying pretrained model is at risk, such as lacking robustness to adversarial examples, this trending practice of pretraining and fine-tuning also signifies the immediate damage to all downstream tasks. To address this emerging challenge, we propose a novel framework named \textit{SynBench} to evaluate the quality of pretrained representations, in terms of quantifying the tradeoff between standard accuracy and adversarial robustness to input perturbations. Specifically, SynBench 
uses synthetic data generated from a conditional Gaussian distribution to establish a reference characterizing the robustness-accuracy tradeoff based on the Bayes optimal linear classifiers. Then, SynBench obtains the representations of the same synthetic data from the pretrained model and compare them to the reference for performance benchmarking. Finally, we define the ratio of area-under-curves in robustness-accuracy characterization as a quantifiable metric of the quality of pretrained representations. The entire procedure of SynBench is illustrated in Figure \ref{fig:SynBench}.  

Our SynBench framework features the following key advantages. 


\begin{enumerate}[leftmargin=*]
    \item \textit{Soundness}: We formalize the fundamental tradeoff in robustness and accuracy of the considered conditional Gaussian model and use this characterization as a reference to benchmark the quality of pretrained representations.
    \item \textit{Task-independence}: Since the pretraining of large models is independent of the downstream datasets and tasks (e.g., through self-supervised or unsupervised training on broad data at scale), the use of synthetic data in SynBench provides a task-agnostic approach to evaluating pretrained representations without the knowledge of downstream tasks and datasets.
    \item \textit{Completeness and privacy}: The flexibility of generating synthetic data (e.g., by adopting a different data sampling procedure) offers a good proxy towards a more comprehensive evaluation of pretrained representations when fine-tuned on different downstream datasets, especially in the scenario when the available datasets are not representative of the entire downstream datasets. Moreover, the use of synthetic data enables full control and simulation over data size and distribution, protects data privacy, and can facilitate model auditing and governance.
\end{enumerate}

We highlight our \textbf{main contributions} as follows.
\begin{itemize}[leftmargin=*]
    \item We propose SynBench, a novel task-agnostic framework that uses synthetic data to evaluate the quality of pretrained representations. The evaluation process of SynBench is independent of the downstream datasets and tasks and it applies to any model taking continuous data inputs.
    \item Evaluated with several pretrained vision transformers, our experimental results show that the metric provided by SynBench well matches the model performance in terms of adversarial robustness and standard accuracy when finetuned on several downstream datasets. For example, SynBench-Score suggests that the Imagenet21k pretrained network (\textit{ViT-B/16-in21k}) improves with finetuning on Imagenet1k (\textit{ViT-B/16}), echoing with the higher CIFAR10 and CIFAR10-c linear probing accuracy of \textit{ViT-B/16}.
    % \textcolor{orange}{Mention some example?}
    \item We show that SynBench can be used to inform the design and selection of the hyperparameters in robust linear probing to mitigate the robustness-accuracy tradeoff when fine-tuned on downstream datasets. For example, conducting $\epsilon$-robust linear probing with $\epsilon$ selected by SynBench-Score gives \textit{ViT-L/16} $0.2\%$ increase in CIFAR10 accuracy and $1.1\%$ increase in CIFAR10-c accuracy.
    % \textcolor{orange}{Mention some example?}
\end{itemize}


%offers a task-agnostic approach for 

%Why use synthetic data:

%data privacy

%we can benchmark performance wrt to ideal settings (aka remove data bias when sampled from ideal distribution)

%high correlation of model ranking when compared to groundtruth data?

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{figs/system_score_.png}
    \caption{Overview of our SynBench framework. Step 1: generate class conditional Gaussian and form the inputs to the pretrained model; Step 2: gather rendered representations; Step 3: measure and plot the expected bound under a range of threshold accuracy for both input raw data and representations according to~\eqref{eqn:goal}; Step 4: calculate SynBench score by the relative area under curve of the representations to the input data in the expected bound-threshold accuracy plot. 
    % \PYB{If we go by steps, we need to number them in the plot as well} \PYB{Add ``='' in score}
    % \pd{needs a detailed description of the system}
    }
    \label{fig:SynBench}
    \vspace{-1em}
\end{figure}

\vspace{-0.5em}

==> SynBench arxiv/CP_Methodology.tex <==
\section{SynBench: Methodology and Evaluation}
% \vspace{-0.5em}
Without the knowledge of the downstream tasks and data, we aim to develop a task-agnostic framework to evaluate some fundamental behaviors of the representation network. As robustness is a key desired property, we probe the network to check how representation networks are preserving robustness in the original data. 
It is crucial to note that the probing method developed herein specifies the robustness-accuracy tradeoff in the pretrained representations, can be used for understanding (and possible ranking) different pretrained networks.
% should serve as a fast check of the representation networks and is not sufficient to rank representation networks. \PYB{This sentence seems weak; can we tweak it to say our quantification specifies the robustness-accuracy tradeoff in the pretrained representations, can be used for understanding (and possible ranking) different representation networks}

On the whole, we want to measure the idealized robustness-accuracy tradeoff using synthetic data. By propagating the Gaussian realizations through different representation networks, we can also measure the robustness-accuracy tradeoff for representations. We start this section by giving the synthetic data of interest.


\subsection{Linear Classifier}
We consider binary classification problems with data pair $(x, y)$ generated from the mixture of two Gaussian distributions 
\begin{align}
    x|y \sim \mathcal{N}(y\mu, \Sigma), \label{eqn:symmetric_gaussian}
\end{align} 
where $y\in\mathcal{C}=\{+1, -1\}$, $P(y=+1)=\varProb$, and $P(y=-1)=1-\varProb$. When sampling from this idealized distribution, we eliminate the factor of data bias and can benchmark the robustness degradation in an ideal setting. 
% \PYB{I think we need a few sentences to describe what is adversarial robustness to input perturbations (consistent top-1 prediction) and certified radius and so on} \PYB{We also need to formally introduce the definition of Bayes optimal classifier}

For a given classifier $f$ and input $x$ with $f(x)=y$, where $y$ is the predicted label, it is not rational for the classifier to respond differently to $x+\delta$ than to $x$ for a small perturbation level measured by $\|\delta\|_p$, i.e. inconsistent top-1 prediction~\citep{szegedy2013intriguing,goodfellow2014explaining}. Therefore, the level of (adversarial) robustness for a classifier can be measured by the minimum magnitude of perturbation that causes misclassification, i.e. $\min_{\delta: f(x+\delta)\neq f(x)} \|\delta\|_p$. 
% \PYB{This is not true; are U trying to say eps ball? or not equal?} 
For a generic function $f$, solving the optimization problem exactly is hard~\citep{katz2017reluplex,sinha2018certifying}. 
Luckily, one can readily solve for the optimization if $f$ is affine~\citep{moosavi2016deepfool}. 

In the following, we will exploit this point and consider the linear classifier that minimizes the robust classification error. An ideal candidate classifier for the class conditional Gaussian (\eqref{eqn:symmetric_gaussian}) is specified by the robust Bayes optimal classifier~\citep{bhagoji2019lower,dobriban2020provable}. Specifically, it is stated that the optimal robust classifier (with a robust margin $\epsilon$) for data generated from~\eqref{eqn:symmetric_gaussian} is a linear classifier $f(x)=sign(w_0^Tx)$, where $w_0=\Sigma^{-1}(\mu-z_\Sigma(\mu))$, $z_\Sigma(\mu)=\argmin_{\|z\|_2\leq \epsilon} (\mu-z)^T \Sigma^{-1} (\mu-z)$, and $sign(\cdot)$ is the typical sign function. 
To simplify the exposition, we focus on $\ell_p$ with $p=2$ in the remainder of this paper\footnote{We put Bayes optimal $\ell_\infty$ robust classifier in the appendix~\ref{appendix:l_inf}.}.
% \PYB{Need to defing sign function} 
We derive the following result as a direct application of the fact:
% follows A direct result of this fact is as follows: \PYB{Not clear this is our result or known result; if it's the latter, need to cite}
% Thus, two streams of methods are developed to either derive the lower bound, or the upper bound, of the exact solution of $\max_{f(x+\delta)=f(x)} \|\delta\|_p$. Given an input $x$, a classifier $f$, and their induced lower bound of $\max \|\delta_x\|_p$, $\text{lwb}(\max \|\delta_x\|_p)$, we say the network is \textit{certifiably robust} to perturbations under $\ell_p$ attack model up to $\text{lwb}(\max \|\delta_x\|_p)$. In the evaluation of pretrained representations, we are dedicated to give the ceritified lower bound given the representations and the optimal (robust) Bayes classifier.

\begin{theorem}
For samples $x$ following the conditional Gaussian in~\eqref{eqn:symmetric_gaussian} with $\Sigma= I_\varDimension$ ($d$ by $d$ identity matrix)
% \PYB{Need to define identity matrix}
, given an $\ell_2$ adversarial budget $\epsilon\leq \|\mu\|_2$, the robust Bayes optimal classifier has the decision margin $\delta$ lower bounded by $\frac{\lvert q/2 - x^T \mu(1-\epsilon/\|\mu\|_2) \rvert}{(1-\epsilon/\|\mu\|_2)\|\mu\|_2}$, where $q=ln\{(1-\varProb)/\varProb\}$. With $\varProb=\frac{1}{2}$, the lower bounds become $\frac{\lvert x^T \mu\rvert}{\|\mu\|_2}$.
\end{theorem}
Since the bound is subject to the distance between two Gaussians, we scale the bound by $\|\mu\|$ and obtain the minimal scaled perturbation $\bar{\delta}$ as
\begin{align*}
    \|\bar{\delta}\|_2 \geq \frac{\lvert x^T \mu\rvert}{\|\mu\|^2_2}.
\end{align*}
We note that when the classes are balanced, for samples generated from~\ref{eqn:symmetric_gaussian} and $\Sigma=\sigma^2I_\varDimension$, all $\epsilon$-robust Bayes optimal classifier overlap with each other. However, for data generated from conditional Gaussian with general covariance matrices,  the $\epsilon$ of a $\epsilon$-robust Bayes classifier specifies the desired size of margin and demonstrates the robustness accuracy tradeoff (see Figure~\ref{fig:tradeoff}). 
\begin{figure}[t]
    \centering
    \begin{subfigure}[2D Gaussian case]{
        \includegraphics[width=0.45\textwidth]{figs/2d.png}
        \label{fig:gaussian}}
    \end{subfigure}
    \begin{subfigure}[Theoretical robustness-accuracy tradeoff]{
        \includegraphics[width=0.48\textwidth]{figs/plot_accuracy_mu_0922_tradeoff.png}
        % \caption{The theoretically characterized robustness-accuracy tradeoff.}
            \label{fig:theo_tradeoff}}
    \end{subfigure}
    % \begin{subfigure}[accuracy]{
    %     \includegraphics[width=0.31\textwidth]{figs/acc.png}
    %     \label{fig:tradeoff_acc}}
    % \end{subfigure}
    % \begin{subfigure}[expected bound]{
    %     \includegraphics[width=0.31\textwidth]{figs/bnd.png}
    %     \label{fig:tradeoff_bound}}
    % \end{subfigure}
    \caption{Illustration of robustness-accuracy tradeoff suggested by $\epsilon$-robust Bayes optimal classifiers. Figure (a) depicts a class conditional 2D Gaussian case with decision boundaries drawn by $\epsilon$-robust Bayes optimal classifiers of varying $\epsilon$ values. Figure (b) draws the theoretically characterized robustness-accuracy tradeoff given in Result~\ref{thm:raw_expected_bound}.
    % Figure (b) and (c) exemplify the accuracy and expected bounds induced by $\epsilon$-robust Bayes optimal classifiers on representations. \PYB{May add more details or ref to experiments on what representations they are}
    }
    \label{fig:tradeoff}
\end{figure}

\subsection{Objective}
For a given representation network, we are interested in evaluating the expected bounds under a thresholding accuracy $a_{t}$, i.e. $\mathbb{E}_{\mu\sim \mathbb{P}_\mu, \Sigma\sim \mathbb{P}_\Sigma, x-\bar{\mu}|y \sim \mathcal{N}(y\mu, \Sigma)}\left[\|\bar{\delta}\|_2 \mid \hat{y}^*(x)=y, a>a_{t} \right]$, where $\mathbb{P}_\mu$ and $\mathbb{P}_\Sigma$ characterize the probability density function of the synthetic data manifold of interest, and $\bar{\mu}$ is a translation vector allowing non-symmetric class conditional Gaussian. Here, without the prior of applications, we assume $\mu=s\cdot 1_\varDimension/\sqrt{\varDimension}$, where $s$ denotes a random variable that follows uniform distribution and $1_\varDimension/\sqrt{\varDimension}$ is the normalized all-ones vector. For simplicity, we let $\Sigma=I_\varDimension$. Formally, we define $E_{\theta,\epsilon}(a_{t})$ as 
% \jeet{Maybe skip the introduction of $\mathbb{P}_\Sigma$ and directly give the value of $\Sigma$ you use in the rest of the paper. Similarly for $\mathbb{P}_\mu$, define $s$ with some motivations. Currently it is not clear why such an $s$ is useful.}
\begin{align}
    E_{\theta,\epsilon}(a_{t})=&\mathbb{E}_{s, x}\left[\|\bar{\delta}\|_2 \mid \hat{y}^*(x)=y, a>a_{t}, \mu=s\cdot 1_\varDimension/\sqrt{\varDimension}, \Sigma=I_\varDimension \right]\nonumber\\ 
    =&\sum_i\mathbb{E}_{ x}\left[\|\bar{\delta}\|_2 \mid \hat{y}^*(x)=y, a>a_{t}, \mu=s_i\cdot 1_\varDimension/\sqrt{\varDimension}, \Sigma=I_\varDimension \right]\mathbb{P}(s=s_i)\nonumber\\
    =&\frac{1}{n}\sum_i\mathbb{E}_{ x}\left[\|\bar{\delta}\|_2 \mid \hat{y}^*(x)=y, a>a_{t}, \mu=s_i\cdot 1_\varDimension/\sqrt{\varDimension}, \Sigma=I_\varDimension \right]\nonumber\\
    =&\frac{1}{n}\sum_i\mathbb{E}_{ x-\bar{\mu}|y\sim \mathcal{N}(y s_i\cdot 1_\varDimension/\sqrt{\varDimension}, I_\varDimension)} \left[\|\bar{\delta}\|_2 \mid \hat{y}^*(x)=y \right]\mathbbm{1}_\mathrm{a(s_i\cdot 1_\varDimension/\sqrt{\varDimension},I_\varDimension, \epsilon)>a_{t}},\label{eqn:goal}
\end{align}
where $\mathbbm{1}_\mathrm{a(s_i\cdot 1_\varDimension/\sqrt{\varDimension},I_\varDimension, \epsilon)>a_{t}}$ is the indicator function specifying the $s_i,\epsilon$-dependent $a$ that surpasses the threshold accuracy $a_t$.
In the following sections, we will illustrate how to calculate the inner expectation term $\mathbb{E}_{ x-\bar{\mu}|y\sim \mathcal{N}(y s_i\cdot 1_\varDimension/\sqrt{\varDimension}, I_\varDimension)} \left[\|\bar{\delta}\|_2 \mid \hat{y}^*(x)=y \right]$ for both the raw data and representations. 
% \PYB{Define indicator function}

\subsubsection{Raw data}
Denote the CDF of the standard normal distribution as $\Phi$, we rely on the below two theorems to obtain the expected bounds for the generated synthetic data:

\begin{theorem}
Assume a balanced dataset ($\varProb=\frac{1}{2}, q=0$) where samples $x$ follow the general conditional Gaussian $x|y=1 \sim \mathcal{N}(\mu_1, \Sigma),x|y=-1 \sim \mathcal{N}(\mu_2, \Sigma)$, given an $\ell_2$ adversarial budget $\epsilon$, the robust Bayes optimal classifier gives a standard accuracy of $\Phi(\frac{\tilde{\mu}^T \Lambda^{-1}(\tilde{\mu}-z_{\Lambda}(\tilde{\mu}))}{\|\Lambda^{-1}(\tilde{\mu}-z_{\Lambda}(\tilde{\mu}))\|_{\Lambda}})$, where $\tilde{\mu}=F^T\frac{\mu_1-\mu_2}{2}$, $F\Lambda F^T=\Sigma$ is the economy-size (thin) decomposition with nonzero eigenvalues, and $z_{\Lambda}$ is the solution of the convex problem $\argmin_{\|z\|_2\leq \epsilon} (\mu-z)^T \Lambda^{-1} (\mu-z)$.
\label{thm:raw_expected_accuracy}
\end{theorem}

% \PYB{Define $\Phi$}

While Result~\ref{thm:raw_expected_accuracy} gives us the theoretical classification accuracy as a function of synthetic conditional Gaussian parameters, the following result establishes a direct link between the expected scaled bound and accuracy (i.e. robustness-accuracy tradeoff).

\begin{theorem}
Assume a balanced dataset ($\varProb=\frac{1}{2}, q=0$) where samples $x$ follow the general conditional Gaussian $x|y=1 \sim \mathcal{N}(\mu_1, \Sigma),x|y=-1 \sim \mathcal{N}(\mu_2, \Sigma)$, given an $\ell_2$ adversarial budget $\epsilon$, the robust Bayes optimal classifier gives an expected scaled bound of $\mathbb{E}\left[\|\bar{\delta_x}\|_2 \mid \hat{y}^*(x)=y\right] \geq  \frac{1}{\sqrt{2\pi}}\frac{1}{a\Phi^{-1}(a)}e^{-\frac{1}{2}\left(\Phi^{-1}(a)\right)^2} + 1$, where $a$ denotes the standard accuracy.
\label{thm:raw_expected_bound}
\end{theorem}

% \begin{wrapfigure}{r}{0.5\textwidth}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figs/plot_accuracy_mu_0922_tradeoff.png}
%     \caption{The theoretically characterized robustness-accuracy tradeoff.}
%     \label{fig:theo_tradeoff}
% \end{wrapfigure}

The subscript $x$ in the expected scaled bound $\mathbb{E}\left[\|\bar{\delta_x}\|_2\mid \hat{y}^*(x)=y\right]$ indicates the raw data space, to distinguish from the scaled bound to be derived for representations.
We highlight that Result~\ref{thm:raw_expected_bound} directly gives a robustness-accuracy tradeoff. We plot the expected scaled bound as a function of accuracy in Figure~\ref{fig:theo_tradeoff}. This tradeoff holds true when the data follow the conditional Gaussian exactly. 
In the proposed SynBench framework, we treat this theoretically-derived robustness-accuracy tradeoff as the reference, enabling a fair comparison among representations induced by different pretrained models. 
% \PYB{We should highlight this is the ``reference'' we mentioned echoing the Intro and Abstract}
We give an illustrative 2D class conditional Gaussian example in Figure~\ref{fig:gaussian}, where different $\epsilon$-robust Bayes classifiers give different overall margins at the cost of accuracy. Concretely, as the $\epsilon$ increases, robust Bayes optimal classifier rotates counterclockwise, leading to misclassifications, but overall bigger margins. 
% For data that do not follow the conditional Gaussian exactly, $\epsilon$-robust Bayes optimal classifier also empirically gives a robustness-accuracy tradeoff as in Figure~\ref{fig:tradeoff_acc} and \ref{fig:tradeoff_bound}.

By now, with Result~\ref{thm:raw_expected_bound}, we can already calculate the inner expectation term in~\eqref{eqn:goal} for the raw data and provide a theoretically-sounded characterization of  robustness-accuracy tradeoff of Bayes optimal classifiers on raw data.

\subsubsection{Representations}
Given a pretrained network 
% \pd{use of two representations in this sentence is confusing, replace the first one with pre-trained network}
, we gather the representations of the Gaussian realizations and quantify the desired bound induced by robust Bayes optimal classifier in the representation space. When deriving the robust Bayes optimal classifier, we model the representations by a general conditional Gaussian $z|y=1 \sim \mathcal{N}(\mu_1, \Sigma),z|y=-1 \sim \mathcal{N}(\mu_2, \Sigma)$. It is worthwhile to note that now the Bayes optimal classifier does not necessarily coincide with robust Bayes optimal classifier even when the dataset is class balanced (see Figure~\ref{fig:gaussian}). The following result is essential to the development of the robustness-accuracy quantification of representations.
\begin{theorem}
For representations $z$ following the general class-balanced conditional Gaussian $z|y=1 \sim \mathcal{N}(\mu_1, \Sigma),~~z|y=-1 \sim \mathcal{N}(\mu_2, \Sigma)$, given an $\ell_2$ adversarial budget $\epsilon$, the robust Bayes optimal classifier has the decision margin $\delta_z$ lower bounded by $\frac{\lvert  (z-\frac{\mu_1+\mu_2}{2})^T F\Lambda^{-1}(\tilde{\mu}-z_{\Lambda}(\tilde{\mu})) \rvert}{\|F\Lambda^{-1}(\tilde{\mu}-z_{\Lambda}(\tilde{\mu})) \|_2}$, and a scaled bound of $\|\bar{\delta_z}\|_2\geq \frac{\lvert  (z-\frac{\mu_1+\mu_2}{2})^T F\Lambda^{-1}(\tilde{\mu}-z_{\Lambda}(\tilde{\mu})) \rvert}{\lvert \tilde{\mu}^T\Lambda^{-1}(\tilde{\mu}-z_{\Lambda}(\tilde{\mu}))\rvert}$, where $\tilde{\mu}=F^T\frac{\mu_1-\mu_2}{2}$, $F\Lambda F^T=\Sigma$ is the  economy-size (thin) decomposition with nonzero eigenvalues, and $z_{\Lambda}$ is the solution of the convex problem $\argmin_{\|z\|_2\leq \epsilon} (\mu-z)^T \Lambda^{-1} (\mu-z)$.
\label{thm:rep_bound}
\end{theorem}

% \PYB{1 seems not a professional notation}

\subsection{Robustness-Accuracy Quantification of Representations}
\label{subsec:metrics}
Recall that we want to calculate $$E_{\theta,\epsilon}(a_{t})=\frac{1}{n}\sum_i\mathbb{E}_{ x|y\sim \mathcal{N}(y s_i\cdot 1_\varDimension/\sqrt{\varDimension}, I_\varDimension)} \left[\|\bar{\delta}\|_2 \mid \hat{y}^*(x)=y \right]\mathbbm{1}_\mathrm{a(s_i\cdot 1_\varDimension/\sqrt{\varDimension},I_\varDimension, \epsilon)>a_{t}}$$ for both raw data and the representations (i.e. $\|\bar{\delta_x}\|$ and $\|\bar{\delta_z}\|$).
We treat the expected bounds of the raw data under a threshold accuracy as the reference. Given a representation network, we compare the expected bounds of the representations rendered by representation networks with the reference.

We take $s\sim \mathcal{U}\{0.1,5\}$ under the guidance of Result~\ref{thm:raw_expected_accuracy}. Specifically, as Results~\ref{thm:raw_expected_accuracy} gives an analytical expected accuracy for class conditional Gaussian, we can obtain the desired range of $s$ by giving the accuracy. Now since we are interested in having the reference as a class conditional Gaussian that yields accuracy from 55\% to almost 100\%, we set the starting and ending $s$ by the fact that $\Phi(0.1) \sim 0.55$ and $\Phi(5) \sim 1.0$.
We reiterate that with more accurate modelling of the data manifold of interest, SynBench can give more precise capture of the pretrained representation performance.
% \jeet{Mention the fact that $\Phi(0.1) \sim 0.5$ and $\Phi(5) \sim 1.0$. Currently the values seem arbitrary.}

When the data is perfect Gaussian (e.g. raw data), we calculate $E_{\theta_\raw,\epsilon}(a_{t})$ with the help of Result~\ref{thm:raw_expected_bound}. Since $E_{\theta_\raw,\epsilon}(a_{t})$ of the raw data is defined for a specific representation network parameter $\theta_\raw$, and all the $\epsilon$-robust classifiers overlap with each other, we further denote it by $E(a_{t})$ to differentiate it from that of the representations. 
For representations, we calculate $E_{\theta,\epsilon}(a_{t})$ with the help of Result~\ref{thm:rep_bound} and the expectation is estimated empirically.
We show an example of the probing results in Figure~\ref{fig:threshold_accu}.
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{figs/threshold_AUC_marker_straight.png}
    \caption{An example of the robustness-accuracy quantification of representations for ViT-B/16. (Left) The expected bound as a function of the threshold accuracy, $E(a_{t})$ and $E_{\theta,\epsilon}(a_{t})$, for $\epsilon=0\sim0.8$. (Right) The desired quantification SynBench-Score$(\theta,\epsilon,a_{t})=\frac{\text{area B}}{\text{area A} + \text{area B}}$ (refer to~\eqref{eqn:SynBench_Score}) for $\epsilon=0$ (top) and $\epsilon=0.6$ (bottom).}
    \label{fig:threshold_accu}
\end{figure}

To integrate over all the desired threshold accuracy, we use the area under the curve (AUC) and give the ratio to the reference by 
\begin{align}
    \text{SynBench-Score}(\theta,\epsilon,a_{t}) =  \frac{\int^1_{a_{t}}E_{\theta,\epsilon}(a)da}{\int^1_{a_{t}}E(a)da},\label{eqn:SynBench_Score}
\end{align}
which correspond to $\frac{\text{area B}}{\text{area A + area B}}$ in Figure~\ref{fig:threshold_accu}. Larger value of SynBench-Score implies better probing performance on pretrained representations.
% Apart from $SynBench(\theta,\epsilon,a_{t})$, we also calculate the average max accuracy (Avg. Max $a$), which is defined by $\text{mean}_{\epsilon}(\max_{\{a_t: E_{\theta,\epsilon}(a_{t})>0\}}a_t)$. We note that this value corresponds exactly to the average ``vanishing accuracy'' as shown in Figure~\ref{fig:threshold_accu}. As the ``vanishing accuracy'' gives an intuitive sense of the separability of representations rendered by the network, different $\epsilon$-robust Bayes classifier further offers a good proxy to possible downstream classifiers. By taking the average over $\epsilon$, we expect to have an initial capture of the representation quality. 

% \jeet{Motivate the metric average max accuracy a bit more. Try to have a one line equation defining the metric if possible. Its hard to notice a new metric is defined in this paragraph.}

==> SynBench arxiv/CP_RelatedWork.tex <==
\section{Related Work}
% \vspace{-0.5em}
\textbf{Pretrained models in vision.}
In the past few years, much focus in the machine learning community has been shift to train representation networks capable of extracting features for a variety of downstream tasks with minimal fine-tuning.
Nowadays, many common vision tasks are achieved with the assistant of good backbones, e.g. classifications~\citep{yu2022coca,wortsman2022model,foret2020sharpness,xie2020self,dosovitskiy2020image,Chen2020Generative}, object detection~\citep{redmon2017yolo9000,liu2016ssd}, segmentation~\citep{chen2017rethinking,xie2021segformer}, etc.
Among the popular backbones, vision transformers (ViT)~\citep{dosovitskiy2020image} have attracted enormous interest. 
ViTs stem from Transformers~\citep{vaswani2017attention} and split an image into patches, which are then treated as tokens as for the original Transformers.
We will exemplify the use of SynBench using several pretrained ViTs.

\textbf{Benchmarking pretrained models.}
Since pretrained models are used as a foundation for different downstream tasks, it is central to transfer learning~\citep{neyshabur2020being,pruksachatkun2020intermediate}, and also tightly related to model generalization~\citep{qiao2020learning,carlucci2019domain}.
To benchmark the performance of a pretrained model, it is a convention to apply the pretrained model for a number of popular tasks and conduct linear probing on the representations~\citep{chen2020simple,dosovitskiy2020image,Chen2020Generative,chen2021vision}. Besides linear probing,  evaluation frameworks have been proposed  based on mutual information~\citep{bachman2019learning} and minimum description length (MDL)~\citep{blier2018description,voita2020information}, which are reliant on the label information of the downstream tasks and are hence task-specific. Moreover, recent work~\citep{whitney2020evaluating} also discussed the sensitivity of validation accuracy (nonlinear probes) and MDL to evaluation dataset size, and proposed a variant of MDL and a sample complexity based quantifier that depends on the data distribution. 

It was not until recently that more fundamental questions are brought up related to the pretrained models~\citep{bommasani2021opportunities,tran2022plex,zhang2022contrastive}.
Lately,~\citet{bommasani2021opportunities} raised practical concerns about the homogenization  incentivized by the scale of the pretraining. 
Although the homogenization might help in achieving competitive performance for some downstream tasks, the defects are also inherited by all these downstreams. On that account, a more careful study of the fundamentals of pretrained models is of paramount importance.
~\citet{tran2022plex} was dedicated to explore the reliability of pretrained models by devising 10 types of tasks on 40 datasets in evaluating the desired aspect of reliability. 
Furthermore, it is pointed out by~\citet{zhang2022contrastive} that pretrained models may not be robust to subpopulation or group shift as shown in 9 benchmarks.
The adversarial robustness is benchmarked by authors of~\citep{shao2021adversarial,paul2022vision}, where~\citet{paul2022vision} demonstrated the superior robustness of ViTs through Imagenet and~\citet{shao2021adversarial} conducted white-box and transfer attacks on Imagenet and CIFAR10.

\textbf{Optimal representations.}
In the seminal work of deep representation theory,~\citet{achille2018emergence} depicted the desired optimal representations in supervised learning to be sufficient for downstream task, invariant to the effect of nuisances, maximally disentangled, and has minimal mutual information between representations and inputs. 
Focusing more on generalization than compression,~\citet{dubois2020learning} gave the optimal representation based on $\mathcal{V}$-information~\citep{xu2019theory} and probed generalization in deep learning. More recently,~\citet{ruan2021optimal} defined the optimal representations for domain generalization.
In~\citep{Dubois2022Improving}, authors characterize the idealized representation properties for invariant self-supervised representation learning. Specifically, idealized representation should be well-distinguished by the desired family of probes for potential invariant tasks, have sufficiently large dimension, and be invariant to input augmentations. 

SynBench differs from the above quantifiers as it does not need knowledge of any downstream data and has controls over the evaluation set size since we could draw arbitrary number of synthetic data. With the assumed synthetic data distribution, we could theoretically characterize the robustness-accuracy tradeoff that is independent to the downstream tasks. Therefore, SynBench provides a predefined standard of the tradeoff, which serves as the reference for representations induced by pretrained models. 
It should be also mentioned that, recently \emph{sim-to-real} transfer paradigm has been leveraged to test the quality of real data, by projecting those onto the space of a model trained on large-scale synthetic data generated from a set of pre-defined grammar rules~\citep{marzoev2020unnatural}. SynBench, though conceptually similar at a very high level, is different from that line of work -- as the focus of this work is to quantify the accuracy-robustness tradeoff of pretrained representations using synthetic data from conditional distributions.  
% \paragraph{Bayes optimal classifier.}

% bayes optimal classifier
\vspace{-0.5em}

==> SynBench arxiv/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\varProb}{p}
\newcommand{\varDimension}{d}
\newcommand{\raw}{\text{raw}}
\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

